Uplink Linear Receivers for Multi-cell Multiuser MIMO with Pilot Contamination: Large System Analysis

Base stations with a large number of transmit antennas have the potential to serve a large number of users at high rates. However, the receiver processing in the uplink relies on channel estimates which are known to suffer from pilot interference. In this work, making use of the similarity of the uplink received signal in CDMA with that of a multi-cell multi-antenna system, we perform a large system analysis when the receiver employs an MMSE filter with a pilot contaminated estimate. We assume a Rayleigh fading channel with different received powers from users. We find the asymptotic Signal to Interference plus Noise Ratio (SINR) as the number of antennas and number of users per base station grow large while maintaining a fixed ratio. Through the SINR expression we explore the scenario where the number of users being served are comparable to the number of antennas at the base station. The SINR explicitly captures the effect of pilot contamination and is found to be the same as that employing a matched filter with a pilot contaminated estimate. We also find the exact expression for the interference suppression obtained using an MMSE filter which is an important factor when there are significant number of users in the system as compared to the number of antennas. In a typical set up, in terms of the five percentile SINR, the MMSE filter is shown to provide significant gains over matched filtering and is within 5 dB of MMSE filter with perfect channel estimate. Simulation results for achievable rates are close to large system limits for even a 10-antenna base station with 3 or more users per cell.

==> figures.tex <==
%
\begin{figure}[h]
    \begin{center}
      \includegraphics[width = 4in, clip = true, trim = 10 0 10 0]{Figs/7cellSys.pdf}
      \caption{ In the favourable case, the sum of the received powers of interferers contributing to pilot contamination are very less as compared to that of the desired user. User $1$ in the center cell represents such a scenario. The SINR with a pilot corrupted estimate is then comparable to that of perfect estimate. On the other hand for user $2$ in the center cell, the pilot interferers received powers are comparable to that of the desired user and represents the worst case scenarios.} 
      \label{fig:7cellSys}
    \end{center}
\end{figure}
%
%
%
\begin{figure}[h]
    \begin{center}
      \includegraphics[width = 4in, clip = true, trim = 100 240 90 240]{Figs/m50a1.pdf}
      \caption{ The plot shows the asymptotic SIR of the first user in the first cell when MMSE filter with pilot contaminated estimate is used to decode the received signal along with the baseline comparison criterion of MMSE with a perfect estimate and matched filter with a pilot contaminated estimate for an idealized seven cell set up. It is seen that when the other cell received power is just $10$~dB of that in cell users the MMSE filter with pilot contaminated estimate performs close to its corresponding matched filter. This is because the limitation is now the other cell interference which MMSE filter is not designed to suppress. Hence, we  do not expect the MMSE filter with pilot estimate to be useful when $\beta_j >0.1$ } 
      \label{fig:m50a1}
    \end{center}
\end{figure}
%
%
%
\begin{figure}[h]
    \begin{center}
      \includegraphics[width = 4in, clip = true, trim = 100 240 100 240]{Figs/m50a01.pdf}
      \caption{The plot shows the asymptotic SIR of the first user in the first cell when MMSE filter with pilot contaminated estimate is used to decode along with the baseline comparison criterion of MMSE with a perfect estimate and matched filter with a pilot contaminated estimate for an idealized seven cell set up. In this case when the other cell received powers is $20$~dB lower than that of in-cell received powers significant gains are obtained wit respect using a matched filter with pilot contaminated estimate } 
      \label{fig:m50a01}
    \end{center}
\end{figure}
%
%
%
\begin{figure}[h]
    \begin{center}
      \includegraphics[width = 4in, clip = true, trim = 100 240 100 240]{Figs/AchRate.pdf}
     \caption{The plot shows the sum rate of the users in first cell for different operating points of $\alpha$. The three curves correspond to three different received powers from other cell users. The markers correspond to simulation with $50$-antenna base stations and match the theoretical predictions.} 
      \label{fig:AchRate}
    \end{center}
\end{figure}
%%
\begin{figure}[h]
    \begin{center}
      \includegraphics[width = 4in, clip = true, trim = 100 240 100 240]{Figs/RateDiff.pdf}
      \caption{ The plot shows the loss of rate due to pilot contamination  when an MMSE filter with pilot contaminated estimate is used to decode the received signal as compared to perfect estimate MMSE filter. The different curves correspond to different values of $\alpha$ from $0.2$ to $1$. It is seen that smaller the $\alpha$ the MMSE filter with pilot contaminated estimate performs worse than the ideal MMSE filter. However, the sum rate for users per base station is different.} 
      \label{fig:RateDiff}
    \end{center}
\end{figure}

%%
\begin{figure}[h]
    \begin{center}
      \includegraphics[width = 4in, clip = true, trim = 100 240 100 240]{Figs/VaryAlpha.pdf}
      \caption{ The plot shows the five percentile SIR of the first user in the first cell for a seven cell set up in a non-idealized scenario. The received powers from users can be different depending on their positions and shadowing and hence the received SIR is random. The theoretical curves are matched with simulation. The details are described in section \ref{subsec:FivePer}. } 
      \label{fig:VaryAlpha}
    \end{center}
\end{figure}
